Late Breaking Results: Leveraging Approximate Computing for Carbon-Aware DNN Accelerators

The rapid growth of Machine Learning (ML) has increased demand for DNN hardware accelerators, but their embodied carbon footprint poses significant environmental challenges. This paper leverages approximate computing to design sustainable accelerators by minimizing the Carbon Delay Product (CDP). Using gate-level pruning and precision scaling, we generate area-aware approximate multipliers and optimize the accelerator design with a genetic algorithm. Results demonstrate reduced embodied carbon while meeting performance and accuracy requirements.

==> plots/all_networks_carbon.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions={size 4in,2.2in}]
# Basic settings
set format y '%1.1f'
set yrange [0:1.1]
set ylabel "Normalized Carbon"
set ytics 0, 0.2
set grid lt 1 lc rgb "#eeeeee"
set border

# Style settings
set style data histogram
set style histogram cluster gap 1.2
set style fill solid 0.95 border -1
set boxwidth 0.85

# Legend settings
set key outside horizontal top nobox spacing 0.0 width -1 samplen 2

# X-axis settings
set xtics ("7/14/28\nVGG16" 0.5, "7/14/28\nResNet152" 2.0, "7/14/28\nResNet50" 3.5, "7/14/28\nVGG19" 5.0) \
    scale 0 center offset 0,0.3
set xrange [-0.2:5.7]

# Reference line
set arrow from graph 0, first 1 to graph 1, first 1 nohead lt 2 lc rgb "#999999" lw 0.5

# Plot data
plot 'plots/vgg16.dat' using 2 title 'Exact' lc rgb "#2F2F2F", \
     '' using 3 title 'Approximate' lc rgb "#787878", \
     '' using 4 title 'Proposed' lc rgb "#E65100", \
     'plots/resnet152.dat' using 2 notitle lc rgb "#2F2F2F", \
     '' using 3 notitle lc rgb "#787878", \
     '' using 4 notitle lc rgb "#E65100", \
     'plots/resnet50.dat' using 2 notitle lc rgb "#2F2F2F", \
     '' using 3 notitle lc rgb "#787878", \
     '' using 4 notitle lc rgb "#E65100", \
     'plots/vgg19.dat' using 2 notitle lc rgb "#2F2F2F", \
     '' using 3 notitle lc rgb "#787878", \
     '' using 4 notitle lc rgb "#E65100"
\end{gnuplot}

==> plots/vgg16_trend.tex <==
\begin{gnuplot}[terminal=pdfcairo, terminaloptions={size 4in,3in enhanced}]
set terminal pdfcairo size 4in,3in enhanced font "Times New Roman,13"
set margins 10,2,3,2
set title "7nm - VGG16" offset 0,-0.8 font ",15"
set xlabel "Performance (frames/second)" offset 0,0.3 font ",15"
set ylabel "Manufacturing Carbon (gCO_{2})" offset -0.2,0 font ",15"
set key font ",16"
set xtics font ",13"
set ytics font ",13"
set logscale x
set xrange [1.5:250]
set yrange [0:40]
set arrow from 30, graph 0 to 30, graph 1 nohead lt 1 lw 1 linecolor rgb "#666666"
set arrow from 40, graph 0 to 40, graph 1 nohead lt 1 lw 1 linecolor rgb "#666666"
set arrow from 50, graph 0 to 50, graph 1 nohead lt 1 lw 1 linecolor rgb "#666666"
set label "FPS 30" at 27, graph 0.80 rotate by 90 font ",13"
set label "FPS 40" at 37, graph 0.80 rotate by 90 font ",13"
set label "FPS 50" at 47, graph 0.80 rotate by 90 font ",13"
set label "64 PEs" at 1.5,5.4 offset 1,1 font ",13"
set label "128 PEs" at 3.8,5.5 offset 0,-1 font ",13"
set label "256 PEs" at 7,15.5 offset 0,-1 font ",13"
set label "2048 PEs" at 75,40 offset 0,-1 font ",13"
set key at graph 0.43,0.95 box spacing 0.9 width 1 maxcols 1 
set grid lt 1 lc rgb "#dddddd"
plot \
    'plots/7nm_drop00.dat' using 1:2 title 'Exact' with linespoints pt 7 lc rgb "#004C99" lw 2, \
    'plots/7nm_drop05.dat' using 1:2 title 'Appx 0.5%' with linespoints pt 6 lc rgb "#006400" lw 2, \
    'plots/7nm_drop10.dat' using 1:2 title 'Appx 1%' with linespoints pt 3 lc rgb "#7E1E9C" lw 2, \
    'plots/7nm_drop20.dat' using 1:2 title 'Appx 2%' with linespoints pt 5 lc rgb "#A3333D" lw 2,  \
    'plots/cdp_plot_data.dat' using 1:2 title 'GA-CDP' with points pt 5 lc rgb "#E65100" ps 0.8

\end{gnuplot}

==> related.tex <==
\section{Related Work}\label{sec:related}
